Measuring the performance of investments in information security startups: An empirical analysis by cybersecurity sectors using Crunchbase data

Early-stage firms play a significant role in driving innovation and creating new products and services, especially for cybersecurity. Therefore, evaluating their performance is crucial for investors and policymakers. This work presents a financial evaluation of early-stage firms' performance in 19 cybersecurity sectors using a private-equity dataset from 2010 to 2022 retrieved from Crunchbase. We observe firms, their primary and secondary activities, funding rounds, and pre and post-money valuations. We compare cybersecurity sectors regarding the amount raised over funding rounds and post-money valuations while inferring missing observations. We observe significant investor interest variations across categories, periods, and locations. In particular, we find the average capital raised (valuations) to range from USD 7.24 mln (USD 32.39 mln) for spam filtering to USD 45.46 mln (USD 447.22 mln) for the private cloud sector. Next, we assume a log process for returns computed from post-money valuations and estimate the expected returns, systematic and specific risks, and risk-adjusted returns of investments in early-stage firms belonging to cybersecurity sectors. Again, we observe substantial performance variations with annualized expected returns ranging from 9.72\% for privacy to 177.27\% for the blockchain sector. Finally, we show that overall, the cybersecurity industry performance is on par with previous results found in private equity. Our results shed light on the performance of cybersecurity investments and, thus, on investors' expectations about cybersecurity.

==> backup_tables.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lcccccc}           
Sector & \#firms & \#Rounds & Avg. & Median  & Total & SD \\ \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
Artificial Intelligence & $27,879$ & $18,801$ & $14.21$ & $2$ & $267,126.80$ & $73.76$ \\ 
Biometrics & $687$ & $484$ & $7.84$ & $1.60$ & $3,794.91$ & $22.98$ \\ 
Blockchain & $6,844$ & $4,428$ & $14.56$ & $2$ & $64,468.55$ & $55.94$ \\ 
Cloud Security & $1,565$ & $1,269$ & $19.00$ & $6$ & $24,105.40$ & $40.55$ \\ 
Cyber Security & $6,481$ & $4,609$ & $18.73$ & $5$ & $86,313.70$ & $67.21$ \\ 
%Darknet & $12$ & $11$ & $9.76$ & $0.59$ & $107.40$ & $19.91$ \\ 
E-Signature & $197$ & $152$ & $10.69$ & $1.45$ & $1,624.94$ & $37.05$ \\ 
Facial Recognition & $304$ & $222$ & $18.12$ & $1.66$ & $4,023.40$ & $68.71$ \\ 
Fraud Detection & $939$ & $671$ & $21.23$ & $5$ & $14,247.66$ & $68.91$ \\ 
%Homeland Security & $174$ & $128$ & $6.33$ & $3.05$ & $810.31$ & $7.73$ \\ 
Internet of Things & $9,699$ & $6,416$ & $8.19$ & $1.32$ & $52,543.11$ & $33.06$ \\ 
Intrusion Detection & $99$ & $76$ & $24.30$ & $4.25$ & $1,846.68$ & $62.47$ \\ 
Machine Learning & $17,202$ & $11,669$ & $12.40$ & $2.02$ & $144,683.90$ & $45.17$ \\ 
Network Security & $3,389$ & $2,708$ & $18.36$ & $6.71$ & $49,712.68$ & $71.51$ \\ 
Penetration Testing & $80$ & $58$ & $9.06$ & $2$ & $525.57$ & $20.72$ \\ 
Privacy & $939$ & $648$ & $11.80$ & $3.20$ & $7,649.03$ & $32.63$ \\ 
Private Cloud & $202$ & $163$ & $37.39$ & $10$ & $6,093.76$ & $105.07$ \\ 
QR Codes & $122$ & $93$ & $13.23$ & $0.18$ & $1,230.18$ & $53.50$ \\ 
Quantum Computing & $340$ & $234$ & $15.62$ & $4.64$ & $3,655.45$ & $44.46$ \\ 
Security & $14,582$ & $10,586$ & $14.86$ & $4.10$ & $157,287.70$ & $53.54$ \\ 
Spam Filtering & $31$ & $17$ & $7.14$ & $6$ & $121.39$ & $7.52$ \\ 
Total & $91,767$ & $63,443$ & $14.06$ & $2.50$ & $891,972.50$ & $59.27$ \\ 
\end{tabular}
\caption{\footnotesize{Number of firms and rounds for each cybersecurity sector and descriptive statistics for their funding rounds. The data is from 2010 to 2022}}
\footnotesize{Funding values are in USD mln.}
\label{tab_descr_funding}
\end{table}



\begin{table}[H]
\centering
\begin{tabular}{lcccc}           
Sector & Avg. & Median  & Total & SD \\ \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
Artificial Intelligence     & $712.28$ & $12.56$ & $1,186,663.00$ & $2,527.54$ \\ 
Biometrics                  & $78.32$ & $7.60$ & $2,662.90$ & $224.63$ \\ 
Blockchain                  & $682.39$ & $17.80$ & $404,660.20$ & $1,918.89$ \\ 
Cloud Security              & $793.92$ & $462.50$ & $80,979.47$ & $1,181.06$ \\ 
Cyber Security              & $875.25$ & $88$ & $354,477.30$ & $1,590.70$ \\ 
%Darknet                    & NA & NA & $0$ & NA \\ 
E-Signature                 & $587.74$ & $89.68$ & $13,517.96$ & $948.64$ \\ 
Facial Recognition          & $1,223.09$ & $23$ & $30,577.26$ & $1,905.75$ \\ 
Fraud Detection             & $1,624.57$ & $250$ & $115,344.60$ & $3,948.01$ \\ 
%Homeland Security          & $1.97$ & $1.97$ & $1.97$ & NA \\ 
Internet of Things          & $170.89$ & $5.11$ & $72,113.56$ & $586.86$ \\ 
Intrusion Detection         & $1,334.65$ & $15.90$ & $9,342.57$ & $1,651.33$ \\ 
Machine Learning            & $622.94$ & $12.30$ & $628,550.20$ & $2,162.71$ \\ 
Network Security            & $817.17$ & $100$ & $134,833.50$ & $1,391.23$ \\ 
Penetration Testing         & CHECK & CHECK & CHECK & CHECK \\ 
Privacy                     & $532.79$ & $9$ & $23,975.45$ & $1,369.96$ \\ 
Private Cloud               & $5.45$ & $22.02$ & $2,364.79$ \\ 
QR Codes                    & $314.57$ & $3.85$ & $8,178.79$ & $782.22$ \\ 
Quantum Computing           & $567.25$ & $22.95$ & $7,374.20$ & $1,157.36$ \\ 
Security                    & $655.34$ & $24.52$ & $440,390.40$ & $1,400.83$ \\ 
Spam Filtering              & $7.19$ & $8.30$ & $21.56$ & $1.93$ \\ 
Total                       & $666.92$ & $14.10$ & $3,536,687.00$ & $2,043.47$ \\ 

\end{tabular}
\caption{\footnotesize{Descriptive statistics of the post-money valuations for cybersecurity sectors.}}
\footnotesize{Values are in USD mln.}
\label{tab_descr_pmv}
\end{table}




\begin{table}[H] 
\centering 
 \resizebox{\textwidth}{!}{%
\begin{tabular}{@{\extracolsep{5pt}} lccccccccccccccccccc} 
 & AI & BI & BL & CS & CS & E-S & FR & FD & IoT & ID & ML & NS & PT & PR & PC & QR & QC & S & SF \\ 
Artificial Intelligence &  & $5.42$ & $-0.35$ & $-3.80$ & $-4.01$ & $1.15$ & $-0.84$ & $-2.59$ & $8.88$ & $-1.40$ & $2.66$ & $-2.81$ & $1.86$ & $1.73$ & $-2.81$ & $0.18$ & $-0.48$ & $-0.87$ & $3.72$ \\ 
Biometrics & $-1.90$ &  & $-5.01$ & $-7.22$ & $-7.56$ & $-0.90$ & $-2.17$ & $-4.69$ & $-0.31$ & $-2.27$ & $-4.05$ & $-6.09$ & $-0.42$ & $-2.40$ & $-3.56$ & $-0.95$ & $-2.52$ & $-6.01$ & $0.33$ \\ 
Blockchain & $0.30$ & $2.62$ &  & $-3.13$ & $-3.21$ & $1.24$ & $-0.76$ & $-2.39$ & $6.80$ & $-1.35$ & $2.30$ & $-2.36$ & $1.93$ & $1.80$ & $-2.76$ & $0.24$ & $-0.35$ & $-0.30$ & $3.69$ \\ 
Cloud Security & $2.29$ & $5.71$ & $2.63$ &  & $0.18$ & $2.58$ & $0.18$ & $-0.77$ & $8.92$ & $-0.73$ & $5.44$ & $0.36$ & $3.37$ & $4.20$ & $-2.21$ & $1.02$ & $1.08$ & $3.31$ & $5.51$ \\ 
Cyber Security & $3.79$ & $3.54$ & $3.20$ & $-0.14$ &  & $2.54$ & $0.13$ & $-0.88$ & $9.82$ & $-0.77$ & $5.89$ & $0.22$ & $3.34$ & $4.27$ & $-2.25$ & $0.98$ & $1.01$ & $3.46$ & $5.58$ \\ 
E-Signature & $-0.59$ & $1.13$ & $-0.85$ & $-2.41$ & $-1.47$ &  & $-1.35$ & $-2.63$ & $0.82$ & $-1.75$ & $-0.56$ & $-2.32$ & $0.40$ & $-0.34$ & $-3.05$ & $-0.40$ & $-1.18$ & $-1.37$ & $1.01$ \\ 
Facial Recognition & $0.79$ & $2.95$ & $0.92$ & $-0.26$ & $-0.13$ & $1.22$ &  & $-0.58$ & $2.15$ & $-0.72$ & $1.24$ & $-0.05$ & $1.69$ & $1.32$ & $-2.04$ & $0.68$ & $0.46$ & $0.70$ & $2.21$ \\ 
Fraud Detection & $2.43$ & $4.11$ & $2.79$ & $0.90$ & $0.90$ & $1.83$ & $0.58$ &  & $4.85$ & $-0.40$ & $3.28$ & $0.96$ & $3.20$ & $3.19$ & $-1.87$ & $1.30$ & $1.42$ & $2.35$ & $4.37$ \\ 
Internet of Things & $-6.32$ & $0.23$ & $-7.43$ & $-10.22$ & $-10.86$ & $-0.92$ & $-4.18$ & $-8.48$ &  & $-2.24$ & $-7.16$ & $-7.09$ & $-0.32$ & $-2.68$ & $-3.54$ & $-0.91$ & $-2.53$ & $-10.04$ & $0.56$ \\ 
Intrusion Detection & $1.19$ & $4.26$ & $1.50$ & $1.07$ & $0.72$ & $2.06$ & $0.69$ & $0.37$ & $4.16$ &  & $1.66$ & $0.81$ & $1.99$ & $1.72$ & $-1.20$ & $1.22$ & $1.12$ & $1.31$ & $2.32$ \\ 
Machine Learning & $-2.39$ & $2.21$ & $-2.53$ & $-4.99$ & $-6.95$ & $0.46$ & $-1.85$ & $-4.76$ & $6.56$ & $-2.28$ &  & $-4.15$ & $1.21$ & $0.44$ & $-3.03$ & $-0.15$ & $-1.10$ & $-3.68$ & $2.81$ \\ 
Network Security & $2.75$ & $3.21$ & $2.50$ & $-0.30$ & $-0.22$ & $1.31$ & $0.05$ & $-0.94$ & $9.28$ & $-0.72$ & $5.46$ &  & $3.05$ & $3.49$ & $-2.28$ & $0.90$ & $0.85$ & $2.38$ & $4.91$ \\ 
Penetration Testing & $-0.53$ & $0.39$ & $-0.75$ & $-1.85$ & $-1.09$ & $-0.32$ & $-0.99$ & $-1.34$ & $0.20$ & $-1.78$ & $-0.56$ & $-0.99$ &  & $-0.91$ & $-3.27$ & $-0.67$ & $-1.65$ & $-2.09$ & $0.59$ \\ 
Privacy & $-0.83$ & $2.28$ & $-1.22$ & $-3.91$ & $-2.58$ & $0.37$ & $-1.82$ & $-3.16$ & $2.66$ & $-2.80$ & $-0.33$ & $-2.28$ & $0.63$ &  & $-3.07$ & $-0.25$ & $-1.20$ & $-2.21$ & $2.09$ \\ 
Private Cloud & $3.98$ & $5.80$ & $4.90$ & $4.25$ & $3.40$ & $2.96$ & $2.17$ & $2.39$ & $10.06$ & $1.01$ & $6.81$ & $3.20$ & $2.04$ & $5.28$ &  & $2.43$ & $2.49$ & $2.73$ & $3.59$ \\ 
QR Codes & $-0.13$ & $1.58$ & $-0.23$ & $-1.29$ & $-0.78$ & $0.44$ & $-0.61$ & $-1.08$ & $1.44$ & $-1.24$ & $0.18$ & $-0.69$ & $0.57$ & $0.36$ & $-2.07$ &  & $-0.38$ & $-0.29$ & $1.04$ \\ 
Quantum Computing & $0.29$ & $3.09$ & $0.29$ & $-1.15$ & $-0.70$ & $1.14$ & $-0.46$ & $-1.16$ & $3.33$ & $-1.33$ & $1.08$ & $-0.58$ & $1.09$ & $1.39$ & $-2.83$ & $0.41$ &  & $0.26$ & $2.47$ \\ 
Security & $0.80$ & $2.87$ & $0.31$ & $-2.66$ & $-3.78$ & $0.96$ & $-0.89$ & $-2.93$ & $8.99$ & $-1.53$ & $3.71$ & $-2.82$ & $0.82$ & $1.44$ & $-5.22$ & $0.29$ & $-0.22$ &  & $4.07$ \\ 
Spam Filtering & $-0.40$ & $-0.13$ & $-0.55$ & $-1.20$ & $-0.71$ & $-0.39$ & $-0.66$ & $-0.84$ & $-0.13$ & $-1.13$ & $-0.48$ & $-0.65$ & $-0.37$ & $-0.59$ & $-1.18$ & $-0.47$ & $-0.78$ & $-0.59$ &  \\ 
\end{tabular}}
 \caption{t-tests of equal and unequal variances of funding amount for each category}
 \footnotesize{The lower (upper) diagonal entries are t-statistics for tests of equal (unequal, Welch’s t-test) variances. The values are computed comparing the row-wise to the column-wise entries}
  \label{tab_ttest_funding} 
\end{table}

==> backupstyle.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Package loading section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}

\usepackage{setspace}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{datetime}
\usepackage{rotating}
\usepackage{fancyvrb}
\usepackage[shortlabels]{enumitem}
\usepackage{float}
\usepackage{longtable}
\usepackage[margin=0.7in]{geometry}
\usepackage[multiple]{footmisc}
%\usepackage[longnamesfirst]{natbib}
\usepackage[numbers]{natbib}
\usepackage{epstopdf}
\usepackage[export]{adjustbox} % loads also graphicx
\usepackage{lscape}
\usepackage{tikz}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage[toc]{appendix}%[toc,page] 
\usepackage[countmax]{subfloat}
\usepackage{subcaption}
\usepackage{afterpage}

\usepackage{multirow}
\usepackage{nicefrac}
\usepackage{makecell}
\usepackage{units}
\usepackage{booktabs}
\usepackage{tensor}
\usepackage{chngpage}
\usepackage{chapterbib}
\usepackage{indentfirst} % Indent first sentence of a new section.
\usepackage{comment}
\usepackage{hyperref}
\usepackage[utf8]{inputenc}
\usepackage{tabularx}
\usepackage{tocloft}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commands section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}
\newtheorem{condition}{Condition}
\newtheorem{hyp}{Hypothesis}
\newtheorem{subhyp}{}
\renewcommand\thesubhyp{\alph{subhyp}}

% left fixed width (tabularx package)
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
% center fixed width:
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% flush right fixed width:
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcommand\EatDot[1]{}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\renewcommand*{\thesection}{\arabic{section}} % sections' numbering in Arabic
%\renewcommand*{\thechapter}{\Roman{chapter}} % chapters' numbering in Roman
\newif\ifrhsapp
\rhsappfalse

% Section title format / Put dots after numbers in section headers.
\newcommand{\@seccntformat@section}[1]{%
  \ifrhsapp 
  Appendix 
  \else
  \fi
  \csname the#1\endcsname.\quad
}

\newcommand*{\@seccntformat@subsection}[1]{%
  \csname the#1\endcsname.\quad
}

\newcommand*{\@seccntformat@subsubsection}[1]{%
  \csname the#1\endcsname.\quad
}

\let\@@seccntformat\@seccntformat
\renewcommand*{\@seccntformat}[1]{%
  \expandafter\ifx\csname @seccntformat@#1\endcsname\relax
    \expandafter\@@seccntformat
  \else
    \expandafter
      \csname @seccntformat@#1\expandafter\endcsname
  \fi
    {#1}%
}

\renewcommand{\subsection}{\@startsection
  {subsection}{2}{0mm}{-3.25ex \@plus -1ex \@minus -.2ex}{1.5ex \@plus.2ex}{\normalfont\large\itshape}}

\renewcommand{\subsubsection}{\@startsection
  {subsubsection}{2}{0mm}{-3.25ex \@plus -1ex \@minus -.2ex}{1.5ex \@plus.2ex}{\normalfont\itshape}}

\renewcommand{\figurename}{Fig.}

% Put word "Appendix" before appendix number
\def\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \rhsapptrue
  \renewcommand\thesection{\Alph{section}}%
}

%%reset numbering for equations across chapter, with no chapter number
\renewcommand{\theequation}{\arabic{equation}}

%tocloft package
%\setlength{\cftfigindent}{4em}
%\setlength{\cfttabindent}{4em}
\setlength\cftfignumwidth{4em}
\setlength\cfttabnumwidth{4em}

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\let\oldmarginpar\marginpar

\newcommand{\quotes}[1]{``#1''}
% Number paragraphs and subparagraphs and include them in TOC

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Setting specific section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{tocdepth}{2}
\graphicspath{{images/}}
%\bibliographystyle{main/styles/jfe}
\onehalfspacing% Use 1.5 spacing
\usdate
\setlist{noitemsep}% Reduce space between list items


